SAFT: Structure-aware Transformers for Textual Interaction Classification

Textual interaction networks (TINs) are an omnipresent data structure used to model the interplay between users and items on e-commerce websites, social networks, etc., where each interaction is associated with a text description. Classifying such textual interactions (TIC) finds extensive use in detecting spam reviews in e-commerce, fraudulent transactions in finance, and so on. Existing TIC solutions either (i) fail to capture the rich text semantics due to the use of context-free text embeddings, and/or (ii) disregard the bipartite structure and node heterogeneity of TINs, leading to compromised TIC performance. In this work, we propose SAFT, a new architecture that integrates language- and graph-based modules for the effective fusion of textual and structural semantics in the representation learning of interactions. In particular, line graph attention (LGA)/gated attention units (GAUs) and pretrained language models (PLMs) are capitalized on to model the interaction-level and token-level signals, which are further coupled via the proxy token in an iterative and contextualized fashion. Additionally, an efficient and theoretically-grounded approach is developed to encode the local and global topology information pertaining to interactions into structural embeddings. The resulting embeddings not only inject the structural features underlying TINs into the textual interaction encoding but also facilitate the design of graph sampling strategies. Extensive empirical evaluations on multiple real TIN datasets demonstrate the superiority of SAFT over the state-of-the-art baselines in TIC accuracy.

==> ER.tex <==
\begin{lemma}
Let $\EM \in \mathbb{R}^{m\times n}$ be the incidence matrix of $G$, where $\EM[e_{i,j},v_i]=1$ and $\EM[e_{i,j},v_j]=-1$ for each edge $e_{i,j}\in E$  with two end points $v_i,v_j$, $\EM[e_{i,j},v_x]=0$ if $v_x\neq v_i,v_j$. We have $\LM=\EM^{\top}\EM$.
\begin{proof}
Recall that $\LM =\DM-\AM$. Thus, for any node $v_i\in V$, $\LM_{i,i}=d(v_i)$ and for any edge $(v_i,v_j)\in E$, $\LM_{i,j}=\LM_{j,i}=-1$. For any two nodes $v_i,v_j$ such that $v_i\neq v_j$ and $(v_i,v_j)\notin E$, $\LM_{i,j}=\LM_{j,i}=0$.

for any two nodes $v_i,v_j\in V$, $\EM[v_i]\cdot \EM[v_j]=\sum_{e\in E}{\EM[e,v_i]\cdot \EM[e,v_j]}$. 
By definition, if $v_i=v_j$, we have $\EM[v_i]\cdot \EM[v_j]= d(v_i)$.
Note that if node $v_i$ (resp. $v_j$) is not incident to $e$, $\EM[v_i,e]=0$ (resp. $\EM[v_j,e]=0$). So, if $(v_i,v_j)\notin E$ and $(v_j,v_i)\notin E$, we have $\EM[v_i]\cdot \EM[v_j]=0$. If $(v_i,v_j) \in E$ or $(v_j,v_i) \in E$, $\EM[v_i]\cdot \EM[v_j]=\EM[e_{i,j},v_i]\cdot \EM[e_{i,j},v_j]+\EM[e_{j,i},v_j]\cdot \EM[e_{j,i},v_i]=-1$. Therefore, the lemma is proved.
\end{proof}
\end{lemma}


We define matrix $\QM\in \mathbb{R}^{m\times m}$
\begin{equation}\label{eq:Q}
\QM 
=\EM\LM^{+}\EM^{\top}
\end{equation}

\begin{theorem}
$r(e_{i,j})=\QM[e_{i,j}, e_{i,j}]$ holds for every edge $e_{i,j}\in E$.
\begin{proof}
We first prove $\QM[e_{i,j},e_{i,j}]=r(e_{i,j})$ holds for every edge $e_{i,j}\in E$.

$(\EM\LM^{+})[e_{i,j},v_x]=\EM[e_{i,j}]\cdot \LM^{+}[:,v_x]=\LM^{+}[v_i,v_x]-\LM^{+}[v_j,v_x]$. 

This means $(\EM\LM^{+})[e_{i,j},v_i]=\LM^{+}[v_i,v_i]-\LM^{+}[v_j,v_i]$ and $(\EM\LM^{+})[e_{i,j},v_j]=\LM^{+}[v_i,v_j]-\LM^{+}[v_j,v_j]$.

So $(\EM\LM^{+})[e_{i,j},v_i]-(\EM\LM^{+})[e_{i,j},v_j]=r(e_{i,j})$.
Then $\QM[e_{i,j},e_{i,j}]=(\EM\LM^{+}\EM^{\top})[e_{i,j},e_{i,j}]=(\EM\LM^{+})[e_{i,j},v_i]-(\EM\LM^{+})[e_{i,j},v_j]=r(e_{i,j})$.

The theorem is proved.
\end{proof}
\end{theorem}

By Section 2.2 in \cite{spielman2008graph},
\begin{equation}
\LM=\UM\boldsymbol{\Lambda}\UM^{\top}, \LM^{+}=\UM \boldsymbol{\Lambda}^{-1}\UM^{\top}.
\end{equation}

Let $\UM\boldsymbol{\Sigma}\VM^{\top}$ be the SVD of $\EM^{\top}$. Note that $\UM$ and $\VM$ are semi-unitary matrices, i.e., $\UM^{\top}\UM=\VM^{\top}\VM=\IM$. An interesting observation is that
$\LM=\EM^{\top}\EM = \UM\boldsymbol{\Sigma}\VM^{\top}\VM\boldsymbol{\Sigma}\UM^{\top}=\UM\boldsymbol{\Sigma}^2\UM^{\top}$. So, $\LM^{+}=\UM\frac{1}{\boldsymbol{\Sigma}^2}\UM^{\top}$. So, $\QM=\EM\LM^{+}\EM^{\top}=\VM\boldsymbol{\Sigma}\UM^{\top}\cdot\UM\frac{1}{\boldsymbol{\Sigma}^2}\UM^{\top}\cdot \UM\boldsymbol{\Sigma}\VM^{\top}=\VM\VM^{\top}$.

